Bayesian Statistical Model Checking for Multi-agent Systems using HyperPCTL*

In this paper, we present a Bayesian method for statistical model checking (SMC) of probabilistic hyperproperties specified in the logic HyperPCTL* on discrete-time Markov chains (DTMCs). While SMC of HyperPCTL* using sequential probability ratio test (SPRT) has been explored before, we develop an alternative SMC algorithm based on Bayesian hypothesis testing. In comparison to PCTL*, verifying HyperPCTL* formulae is complex owing to their simultaneous interpretation on multiple paths of the DTMC. In addition, extending the bottom-up model-checking algorithm of the non-probabilistic setting is not straight forward due to the fact that SMC does not return exact answers to the satisfiability problems of subformulae, instead, it only returns correct answers with high-confidence. We propose a recursive algorithm for SMC of HyperPCTL* based on a modified Bayes' test that factors in the uncertainty in the recursive satisfiability results. We have implemented our algorithm in a Python toolbox, HyProVer, and compared our approach with the SPRT based SMC. Our experimental evaluation demonstrates that our Bayesian SMC algorithm performs better both in terms of the verification time and the number of samples required to deduce satisfiability of a given HyperPCTL* formula.

==> nonnest.tex <==
\chapter{Bayesian SMC for Non-nested CSL Verification}
\label{chap:baysmc}
In this section, we formulate the verification problem as a hypothesis
testing problem.
The nested probabilistic operators pose a challenge to statistical
analysis, so, we start with formulae without nested probabilistic
operators, and then extend our analysis to nested operators.


\section{Verifying non-nested formulas}
Verification problem can be formulated as a hypothesis testing
problem.
First, we consider a formula with a single probabilistic operator at
the top, namely, $\varphi = \Pr_{\geq \theta_0}( \varrho)$, where $\varrho$ is a path
formula and does not contain any probabilistic operator $\Pr$ within
it.
We refer to such formulae as \emph{non-nested} formulae.

The satisfaction of the path formula $\varrho$ by a path $\sigma$
depends only on a finite prefix of it, whose length, say $\lenf{\varrho}$,
can be upper bounded, for instance, by the sum of the $k$'s in
$\U^{\leq k}$ operators appearing within $\varrho$.
Hence, the satisfaction of $\varphi$ is a state $s$ can be determined
by considering all paths from $s$ of length $\lenf{\varrho}$, verifying if the path
satisfies $\varrho$, summing up the probabilities of all the paths
that satisfy $\varrho$ and checking if it is $\geq \theta_0$.
Note that whether $\sigma \models \varrho$ can be computed in time linear
in the $\lenf{\varrho}$ and size of $\varrho$.
While the above approach provides a deterministic procedure, it is
highly inefficient because we need to enumerate all paths of length
$\lenf{\varrho}$, which are exponentially many in $\lenf{\varrho}$.

To avoid the exponential blow-up in verification complexity, we turn
to a statistical approach wherein the verification problem is
formulated as a hypothesis testing problem as follows.
Let us consider a sample space $\C$ consisting of all finite paths of $\T$
starting from $s$ up to a given length $\lenf{\varrho}$, and let $\C_\varrho$ be
the set of paths in $\C$ which satisfy $\varrho$.
Recall that the probability associated with a finite path $\path$ is
given by $\prob(\path)$.
A standard random walk on the DTMC will sample from $\C$ such that
$\path$ appears with probability $\prob(\path)$.
Let $Y$ be a random variable on this space, such that $Y(\sigma) =
1$ if $\sigma \models \varrho$, and $0$, otherwise.
Note that $\P[Y = 1] = \prob(\C_\varrho)$.
Hence, $Y$ is a Bernoulli random variable with parameter $\Theta =
\prob(\C_\varrho)$.

Further, to solve the verification problem, does $s \models \varphi = \Pr_{\geq
	\theta_0}( \varrho)$, we don't need the exact value of $\Theta$, but
we need to know whether it is greater than or equal to $\theta_0$.
This is essentially a hypothesis test, where the null hypothesis
is given by $H_0: \Theta \geq \theta_0$ vs the alternative hypothesis
$H_1: \Theta < \theta_0$.
We can use Bayes' test to check if $s \models
\varphi$, that is, $s \models \varphi$ if $H_0$ is accepted by the
Bayes' test and $s \not\models \varphi$ if $H_1$ is accepted by the
Bayes' test.
Theorem \ref{thm1} provides upper bounds on Type 1 and Type II errors.
The Type I error corresponds to the probability that the test
falsely concludes that $s$ does not satisfy $\varphi$, and type II
error to the probability that the test falsely concludes that $s$
satisfies $\varphi$.
Unlike the standard model-checking algorithms~\cite{kwiatkowska2011prism}, where we obtain with probability $1$
whether $s \models \varphi$, here, we can only say with high
probability whether $s \models \varphi$.
However, as we will see in the experimental section, statistical
methods are much faster than traditional state space exploration based
model-checking algorithms.


\begin{algorithm}[h] 
	\vspace{2 mm}
	\KwIn{$s$ - state, $\T$ - $\mc$, $\varphi = \Pr_{\op \theta_0}
          (\rho)$ - non-nested $\csl$ formula, $a$, $b$ - parameters
          for beta prior, $\alpha$, $\beta$ - bound on Type I and Type
          II errors
	}
	\vspace{2 mm}
	\KwOut{Answer if $s \models \varphi$ in $\T$ with confidence
          $\alpha, \beta$ }
	\vspace{2 mm}
	\caption{Bayes$\_$SMC$\_$Base - SMC of a non-nested $\csl$ formula}
	\label{algo:base}
	\SetKw{KwGoTo}{go to}
	\Begin{ 	 
          Set $n = 0$, $m = 0$\\
          Set $\lenf{\varrho}$ to be the depth of $\varrho$\\
          
		\While{True}
		{
			Increment $n$\\
			Generate a (random) path $\sigma$ from state $s$ in
                        $\T$ of length $\lenf{\varrho}$ \\
			\If{$\sigma$ satisfies $\rho$} {
				Increment $m$
			}
				Set $B$ = BayesFactor($\theta_0$, $n$, $m$, $a$, $b$) \\
			\If{$B > \frac{1}{\beta}$}
			{
				\textbf{return} \emph{true}		
			}
			\If{$B < \alpha$}{
				\textbf{return} \emph{false}		
			}	
		}
	
	}		 
      \end{algorithm}

Our algorithm for the non-nested case is summarized in Algorithm
\ref{algo:base}.
Algorithms checks if $\varphi = \Pr_{\op \theta_0} (\rho)$ is
satisfied in a state $s$ of $\T$, under the assumption that the prior
distribution of $\Theta$ is a Beta distribution with parameters $a$
and $b$.
Our algorithm is a randomized algorithm which outputs the correct
answer to $s \models \varphi$ with high probability, that is, the Type
I and II error probabilities are bounded by $\alpha$ and $\beta$.
The algorithm consists of sampling a sequence of paths $\sigma$ of length
$\len{\varrho}$ from $\T$ starting from $s$ and checking if $\sigma
\models \varrho$.
Here, $n$ counts the total number of samples and $m$ counts those that
satisfy $\varrho$.
BayesFactor($\theta_0$, $n$, $m$, $a$, $b$)  computes the
      $B$ as given below, based on which the decision to accept or reject is
      made to ensure Type I and Type II errors are within $\alpha$ and
      $\beta$, respectively, in accordance with Theorem \ref{thm1}.  
\[B = \frac{\P_1}{\P_0}
  *\frac{\int_{\theta_0}^1(\theta)^{m}(1-\theta)^{(n-m)}f_{\Theta}(\theta))d\theta}{\int_0^{\theta_0}(\theta)^{m}(1-\theta)^{(n-m)}f_{\Theta}(\theta)d\theta},
\,\,\,\,\mathrm{where}\,\,
\P_0 = \int_{\theta_0}^1 \f_{\Theta}(\theta)d\theta, 
	\P_1 = \int_0^{\theta_0} \f_{\Theta}(\theta)d\theta\]


  We can summarize the correctness criterion of Algorithm
  \ref{algo:base} as follows:    
      \begin{theorem}
        Let $s$, $\T$, $\varphi$, $a$, $b$, $\alpha$, and $\beta$, be
        as in Algorithm \ref{algo:base}. 
        If $s \models \varphi$ in $\T$, then Algorithm
        \ref{algo:base} outputs true with probability at least $(1 -
        \alpha)$.
         If $s \not\models \varphi$ in $\T$, then Algorithm
        \ref{algo:base} outputs false with probability at least $(1 -
        \frac{1}{\beta})$.
        \end{theorem}



==> recursive.tex <==
\chapter{Bayesian SMC for Nested CSL}
In this section, we extend the Bayesian approach to nested
probabilistic operators.
Bayesian SMC has been explored previously for non-nested
operators~\cite{jha2009bayesian,zuliani2010bayesian}. 
A frequentist SMC approach based on acceptance sampling has been
explored for the complete CSL logic~\cite{younes2002probabilistic}.
Here, we build upon ideas from these papers to address the problem of
Bayesian SMC for the complete CSL logic.


\section{Overview of the approach}
\label{sec:nested}
Standard model-checking algorithms for verifying general CSL formulae
work bottom-up, where the satisfaction of state subformulae are
evaluated at each state, and the satisfaction of a formula containing
these subformulae are inferred from it.
Our broad approach is a similar recursive algorithm, however, there
are several intricacies due to the fact that we can compute the
satisfaction of subformulae exactly using an SMC algorithm.

\begin{figure}
  \begin{center}
  \includegraphics[scale=0.4]{figures/ex1.pdf}
  \caption{$ Pr_{\geq 0.1}(Pr_{\geq 0.2}(F^{\leq 1} b) U^{\leq 4}g)$}
\end{center}
  \label{fig:ex}
\end{figure}

Let us consider a CSL formula $\varphi = \Pr_{\geq \theta_0}(
\varrho)$, where the path formula $\varrho$ could potentially have
probabilistic operators $\Pr$.
We define a top-level formula of $\varrho$, a subformula of $\varrho$
of the form $\Pr_{\geq \theta_0}(\varrho')$ which are not contained
inside any probabilistic operators within $\varrho$.
For instance, consider $\varphi = \Pr_{\geq 0.1} (\varrho)$ where
$\varrho = \psi \ \U^{\leq 4} \  g$ and $\psi =  (\Pr_{\geq 0.2}
\F^{\leq 2} \ b)$ as shown in Figure \ref{fig:ex}.
$\psi$ is a top-level subformula  of $\varrho$.
Suppose $\psi =  (\Pr_{\geq 0.2} \F^{\leq 2} \ \psi')$,
where $\psi' = \Pr_{\geq 0.5}(Xg)$.
Then $\psi'$ would not be a top-level subformula of $\varrho$, since it
is contained within another subformula with a probabilistic operator
at the root, that is, $\psi$, which is a subformula of $\varrho$.

Suppose that we have deduced the satisfaction of all top-level
formulas of $\varrho$ in each state of the DTMC, that is, whether $s
\models \varphi'$ for each state $s$ of the DTMC and each top-level
formula $\varphi'$ of $\varrho$.
Then the verification of $\varphi = \Pr_{\geq \theta_0}(\varrho)$
could be performed as in the case of the non-nested
operators.
That is, given any path $\path$, we can define a random variable $Y$
such that $Y(\path) = 1$ if the $\path$ satisfies $\varrho$, which can
be deduced (computed) deterministically if the values of $s
\models \varphi'$ for each state $s$ and top-level formula $\varphi'$
of $\varrho$ are known.


Again, consider the formula $\varphi$ from Figure \ref{fig:ex}.
The satisfaction of $\varrho$ in a path $\sigma$ depends on the
satisfaction of $\psi$ along states in $\varrho$.
Suppose that we have checked for each state of the DTMC, if $\psi$
holds in that state.
We can then use Algorithm \ref{algo:base} to check if $s \models
\varphi$.
More precisely, we can verify the non-nested formula $\varphi =
\Pr_{\geq 0.1} (p_\psi \ \U^{\leq 4} \  g)$, where the labels of DTMC
now consist of an additional label $p_\psi$ which is added to the
label of exactly those sets that satisfy $\psi$.
Hence, we could verify a nested formula in a bottom up fashion,
provided we can compute the satisfaction of its top-level subformulae
exactly. 

However, our objective is to design a statistical
model-checking algorithm for verifying CSL formulae, and avoid
computationally expensive probabilistic model-checking algorithms.
Hence, we will recursively call SMC algorithms on top-level formulae
$\psi$ of $\varrho$, and use the result in verifying the satisfaction
of $\varrho$.
In this case, the answer to $s \models \psi$ is not definitive,
but has some error given by Type I or Type II errors.
Hence, we need to factor in this uncertain answer for the top-level
subformulae in the analysis of $\varrho$.
We consider a random variable $Z$ such that $Z(\path) = 1$ if $\path$
satisfies $\varrho$ using the values returned by SMC for $s \models
\psi$.
The values of $Z(\path)$ and $Y(\path)$ could differ, since, SMC could
answer the question $s \models \psi$ incorrectly.
However, we can bound probability with which $Z$ differs from $Y$.
This enables us to approximate the Bayes' test based on $Y$, through a
Bayes' test based on $Z$, and use the latter for Bayesian statistical
test for verifying $\varphi$.

Our broad approach consists of the following steps.
\vspace{-0.25cm}
\begin{enumerate}
	\item
	{\bf Recursive step:}
	Compute recursively the $s \models \psi$ for all states $s$ of
        the DTMC $\T$ and	top level formulas $\psi$ of $\varrho$
        using the Bayesian SMC algorithm such that given Type I and
        Type II error bounds, $\alpha_\psi$ and $\beta_\psi$, are
        achieved, respectively. (We assume that the bounds are the
        same for all states, this can be easily relaxed). 
	\item
	{\bf Error Propagation:}
	Propagate the Type I and Type II error bounds, $\alpha_\psi$ and
	$\beta_\psi$ for the top level formulas $\psi$ of $\varrho$ 
	to the root of the formula $\varrho$ to obtain $\alpha_\varrho$ and
	$\beta_\varrho$.
        $\alpha_\varrho$ and $\beta_\varrho$ provide bounds on the Type I
        and Type II errors, $Z$ with respect to $Y$, that is, the
        probability that $\path \models \varrho$ is answered incorrectly
        when SMC results are used for satisfaction of $\psi$ in a
        state as compared to when exact satisfaction answers are used.
       Formally, $\alpha_\varrho$ and $\beta_\varrho$ computed satisfy $\P[Z
       = 0|Y= 1] \leq \alpha_\varrho$ and $\P[Z=1|Y=0] 
	\leq \beta_\varrho$.
	\item
	{\bf Approximate Bayesian Test:}
	While Bayes' test deduces whether $s \models \varphi$ by using
        the values of samples from $Y$, we can only sample values of
        $Z$ using our recursive statistical approach. Hence, we provide an
	approximate Bayesian test, that provides inferences on $s \models
	\varphi$ with given Type I and Type II error guarantees using
        samples of $Z$. 
\end{enumerate}

In Sections \ref{sec:error}  and \ref{sec:test}, we provide the
details of the error propagation step and the approximate Bayesian test, respectively.
In Section \ref{sec:algo}, we present the algorithmic details and
illustrate on an example.


\section{Error Propagation}
\label{sec:error}
In this section, we describe an inductive definition to compute the
Type I and Type II errors, $\typea(\varrho)$ and
$\typeb(\varrho)$, respectively, corresponding to satisfaction of
$\varrho$ (in any path $\path$ of DTMC $\T$) given the Type I and Type
II errors for the SMC of top-level formulae $\psi$ of $\varrho$,
denoted $\typea(\psi)$ and $\typeb(\psi)$, respectively.
In particular, we provide $\typea(\varphi)$ and $\typeb(\varphi)$, for
the case $\varphi = \tt, a, \neg \psi, \psi_1 \land \psi_2$ and $\varrho
= X \psi, \psi_1 \U^{\leq k} \psi_2$.
\begin{itemize}
\item
  $\typea(\tt) =  \typeb(\tt) = 0$;
\item
  $\typea(a) =  \typeb(a) = 0$;
\item
  $\typea(\neg \psi) = \typeb(\psi)$, $\typeb(\neg \psi) = \typea(\psi)$; 
\item
  $\typea(\psi_1 \land \psi_2)  =   \typea(\psi_1)+ \typea(\psi_2)$,
  $\typeb(\psi_1 \land \psi_2) =\max \{  \typeb(\psi_1),
  \typeb(\psi_2)\}$;
\item
  $\typea(X \psi) = \typea(\psi)$, $\typeb(X \psi) = \typeb(\psi)$; 
\item
  $\typea(\psi_1 \U^{\leq k} \psi_2) = k  \typea(\psi_1) + \typea(\psi_2)$,
  $\typeb(\psi_1 \U^{\leq k} \psi_2) = (k+1)\max \{\typeb(\psi_1), \typeb(\psi_2) \}$.
\end{itemize}


% \begin{property} 
% 	\label{r:1} $\\$
% $\star$
% 		$\typea(\neg \psi) = \typeb(\psi)$,  $\typeb(\neg \psi) = \typea(\psi)$; 
% $\star$
% 		$\typea(X \psi) = \typea(\psi)$, $\typeb(X \psi) = \typeb(\psi); \\ $ 
% $\star$
% 		$\typea(\psi_1 \land \psi_2)  =   \typea(\psi_1)+
% 		\typea(\psi_2)$, 
% 		 $\typeb(\psi_1 \land \psi_2) =\max \{  \typeb(\psi_1), \typeb(\psi_2)\}; \\  $ 
% $\star$
% 		$\typea(\psi_1 \U^{\leq k} \psi_2) = k  \typea(\psi_1) + \typea(\psi_2)$,
% 		$\typeb(\psi_1 \U^{\leq k} \psi_2) = (k+1)\max
% 		\{\typeb(\psi_1), \typeb(\psi_2) \}$.
% \end{property}

Below we provide a sketch of correctness of the rules.
Note that the Type I error $\typea(\neg \psi)$ is the probability
that the statistical evaluation of $\neg \psi$ returns false when
it is true. But this is equivalent to the probability of the
statistical evaluation of $\varphi$ returning true when
it is false.
Hence, we obtain $\typea(\neg \psi) = \typeb(\psi)$.
A similar argument provides $\typeb(\neg \psi) = \typea(\psi)$.

$\typea(\psi_1 \land \psi_2)$ is the probability
that the statistical evaluation of $\psi_1 \land \psi_2$ returns false
when it is true.
That is, $\psi_1$ and $\psi_2$ are true but either the statistical
evaluation of $\psi_1$ says false or that of $\psi_2$ says false.
This probability can be upper bounded by the sum of Type I errors
for $\psi_1$ and $\psi_2$.
$\typeb(\psi_1 \land \psi_2)$ is the probability
that the statistical evaluation of $\psi_1 \land \psi_2$ returns true
when it is false.
There are three cases here: $\psi_1$ is true and $\psi_2$ is false,
$\psi_1$ is false and $\psi_2$ is true, and $\psi_1$ and $\psi_2$ are
both false.
Let us consider the case where $\psi_1$ is true and $\psi_2$ is false,
$\psi_1$ is false. The statistical evaluation of $\psi_1 \land
\psi_2$ returns true when the statistical evaluation of $\psi_1$ and
that of $\psi_2$ both return true.
The probability that the statistical evaluation of $\psi_1$ returns true,
when $\psi_1$ is true (and $\psi_2$ is false), is upper bounded by
$1$, while the probability that the statistical evaluation of $\psi_2$ returns true,
when $\psi_2$ is false (and $\psi_1$ is true) is upper bounded by the
Type II error of $\psi_2$.
Hence, the probability that the statistical evaluation of $\psi_1 \land
\psi_2$ returns true, when $\psi_1$ is true and $\psi_2$ is false, is
the product of the above, namely, $1 \times \typeb(\psi_2) = \typeb(\psi_2)$.
Similarly, for the other two cases we can upper bound the probability
by $\typeb(\psi_1)$ and $\typeb(\psi_1) \times \typeb(\psi_2)$.
The overall upper bound is the maximum of all three, namely, $\max \{
\typeb(\psi_1), \typeb(\psi_2)\} $.

Note that $X \psi$ is satisfied by a path $\path$ exactly when $\psi$
is satisfied at $\path[1]$. Hence, the statistical evaluation of $X
\psi$ for $\path$ is incorrect exactly when that of $\psi$ is
incorrect at $\sigma[1]$. Therefore the error probabilities carry
over.
Finally, the Type I and Type II errors for $\psi_1 \U^{\leq k} \psi_2$
are obtained by interpreting $\psi_1 \U^{\leq k} \psi_2$ as the
equivalent formula $\neg \bigwedge_{i = 0}^k  \neg (\bigwedge_{j = 0}^{i-1} X^j
\psi_1 \land X^i \psi_2)$, and using the previous rules.


\section{Approximate Bayesian Test}
\label{sec:test}
In this section, we provide Bayes' test for the verification of a
CSL formula $\varphi = \Pr_{\geq \theta_0}(\varrho)$ on a DTMC $\T$ at
a state $s$, where $\varrho$ could potentially have  probabilistic
operators.
As in the non-nested case, define a random variable $Y$, where
$Y(\sigma) = 1$ if $\sigma$ satisfies $\varrho$, and $0$ otherwise.
Note that $Y$ is a Bernoulli random variable with parameter
$\Theta =\prob(\C_\varrho)$, where $\C_\varrho$ is the set of paths of
$\T$  which satisfy $\varrho$.
For the verification of $\varphi$, we need to test the following hypothesis:
\\
\hspace*{4cm}
$
H_0: \Theta \geq \theta_0  \quad \text{vs} \quad H_1: \Theta<\theta_0
$\\
Ideally, we would like to compute the Bayes' factor $B_Y$ over sampled
data $\y$ consisting of paths starting from the state $s$ and use that
in checking whether the state $s$ satisfies  $\varphi$. 
However, given a path $\sigma$, we cannot check if it satisfies
$\varrho$ exactly, because we do not know the truth values of the nested 
probabilistic operator within $\varrho$ at the different states.
Instead, we have access to an SMC algorithm that deduces the
satisfaction of nested probabilistic operators in the states of DTMC
with certain error bounds.
In Section \ref{sec:error}, we provided the inductive definition to
propagate these errors to $\varrho$.
Hence, we have access to a random variable $Z$ such that $Z(\sigma)$
is $1$ if $\sigma$ satisfies $\varrho$ when SMC values are used for
top-level formulae.
Note that $Z$ will not coincide with $Y$ for a given $\sigma$ always,
but will agree with high probability.
More precisely, we have:
\begin{equation}
\label{eqn:error}
\P[Z=0|Y=1] \leq \alpha_\varrho \ \ \ \ \P[Z=1|Y=0] \leq \beta_\varrho
\end{equation}
Moreover, $Z$ can be interpreted as a Bernoulli random variable with
some parameter $\Theta'$.
Note that in the Bayesian approach, $\Theta$ itself is a random
variable with a sample space $\Omega$.
Our next task is to bound the difference between $\Theta$ and $\Theta'$
(for every point in the sample space for $\Theta$).


\begin{proposition}
\label{prop1}
	Let $Y\sim \Bd(\Theta)$ and  $Z \sim \Bd(\Theta')$ be
        Bernoulli random variables with parameter $\Theta$ and
        $\Theta'$, respectively, and let Equation \ref{eqn:error}
        hold. Then, we have
        $ - \alpha_\varrho \leq \Theta' - \Theta \leq \beta_\varrho$.
\end{proposition}
\begin{proof}
  We know the following facts.
  \begin{itemize}
    \item
  $P[Y= 1] = \Theta, P[Y = 0] = 1 - \Theta,$
  $P[Z= 1] = \Theta', P[Z = 0] = 1 - \Theta'$
  since $Y$ and $Z$ are Bernoulli random variables with parameters
  $\Theta$ and $\Theta'$, respectively;
  \item
  $P[Z=0|Y=1] \leq \alpha_\varrho, P[Z=1|Y=0] \leq \beta_\varrho$,
  from Equation \ref{eqn:error}, and
  \item
$P[Z=1|Y=1] \leq 1, P[Z=0|Y=0] \leq 1$
from the properties of probability measures.
\end{itemize}
We can deduce:
\begin{itemize}
  \item
$\Theta' = P[Z = 1] = P[Z=1|Y=0] P[Y=0] + P[Z=1|Y=1] P[Y=1] \leq \beta_\varrho
(1 - \Theta) + 1. \Theta$
which implies
$\Theta' - \Theta \leq \beta_\varrho  (1 - \Theta) \leq
\beta_\varrho$.
\item
$1 - \Theta' = P[Z = 0] = P[Z=0|Y=0] P[Y=0] + P[Z=0|Y=1] P[Y=1] \leq
1. (1 - \Theta) +  \alpha_\varrho \Theta$
which implies $\Theta' - \Theta \geq - \alpha_\varrho \Theta \geq -
\alpha_\varrho $.
\end{itemize}
\vspace{-0.5in}
\end{proof}

% We establish the relationship between parameter  $\Theta$ for $Y\sim \Bd(\Theta)$ and $\Theta'$ for $Z\sim \Bd(\Theta)$.
% \begin{proposition} 
% 	\label{prop1}
% 	Let $Y\sim \Bd(\Theta)$ and  $Z \sim \Bd(\Theta')$ be Bernoulli random variables with parameter $\Theta$ and $\Theta'$, respectively, and  Equation \ref{eqn:error} hold. Then, we have 
% 	$
% 	 (1-\alpha')\Theta \leq \Theta' \leq \Theta+\beta'(1-\Theta).
% 	 $
% 	% $$ (1-\beta')(1-\theta) \leq \P_{Z|\Theta'}(Z=0|\theta') \leq 1+(\alpha'-1)\theta$$
% \end{proposition} 
% \vspace{-0.10cm}
Next, we present Bayes' test on $Y$ using  Bayes' factor for a test on $Z$ as stated in the following theorem.
\begin{theorem} 	
	\label{thm:yz}
	Let $Y\sim \Bd(\Theta)$ and  $Z \sim \Bd(\Theta')$ be Bernoulli random variables with parameter $\Theta$ and $\Theta'$, respectively, and  Equation \ref{eqn:error} hold. Given hypothesis
	 \[H_0: \Theta \geq \theta_0  \quad \text{vs} \quad H_1:
           \Theta < \theta_0\]
         Consider the test that:
         \begin{itemize}
         \item
           Accepts $H_0$ when $B_{Z}(\z, \theta_0 + \beta_\varrho) \geq
           1/\beta r_1$, and
         \item
           Rejects $H_0$ when $B_{Z}(\z,  \theta_0 - \alpha_\varrho) \leq
           \alpha/r_2$,
         \end{itemize}
         where $B_{Z}$ denotes the Bayes' factor for a test on $Z$,          $r_1 = P[\Theta < \theta_0 + \alpha_\varrho +
           \beta_\varrho]/P[\Theta < \theta_0]$ and
         $r_2 = P[\Theta \geq \theta_0 - \alpha_\varrho -
           \beta_\varrho]/P[\Theta \geq \theta_0]$. Then $\alpha$ and $\beta$
	are  the upper bounds of Type I error and Type II error, respectively.
	\end{theorem}
\begin{proof} First, we show that $\alpha$ is a Type I error bound for
  the hypothesis test, that is, we show that $P(\{\mathrm{reject} \
  H_0\}|H_0) \leq \alpha$.
  
  Note that from Proposition \ref{prop1}, $\Theta(\omega) \geq
  \theta_0$ implies $\Theta'(\omega) \geq \Theta(\omega) - \alpha_\varrho \geq \theta_0 - \alpha_\varrho$.
Hence, 
$\{\omega \,|\, \Theta(\omega) \geq \theta_0\} \subseteq \{\omega \,|\,
\Theta'(\omega) \geq \theta_0 - \alpha_\varrho\}$.
Similarly, $\Theta(\omega) < \theta_0$ implies $\Theta'(\omega) \leq
\Theta(\omega) + \beta_\varrho < \theta_0 + \beta_\varrho$.
Hence, 
$\{\omega \,|\, \Theta(\omega) < \theta_0\} \subseteq \{\omega \,|\,
\Theta'(\omega) < \theta_0 + \beta_\varrho\}$.

Also, from Proposition \ref{prop1}, $\Theta(\omega) \geq
\Theta'(\omega) - \beta_\varrho$. 
Hence, $\Theta'(\omega) \geq \theta_0 - \alpha_\varrho$ implies
$\Theta(\omega) \geq \theta_0 - \alpha_\varrho - \beta_\varrho$. 
Similarly, from Proposition \ref{prop1}, $\Theta(\omega) \leq
\Theta'(\omega) + \alpha_\varrho$.
Hence, $\Theta'(\omega) < \theta_0 + \beta_\varrho$ implies
$\Theta(\omega) < \theta_0 + \beta_\varrho + \alpha_\varrho$. 
\begin{align*}
& P(\{\mathrm{reject} \ H_0\} \ | \ H_0) = P(B_Z(\z, \theta_0 - \alpha_\varrho) \leq \alpha/{r_2} \ | \ H_0) =  P(B_Z(\z, \theta_0 - \alpha_\varrho) \leq \alpha/{r_2}  \ | \ \Theta\geq \theta_0)\\ 
 &=  \frac{P(B_Z(\z, \theta_0 - \alpha_\varrho) \leq \alpha/{r_2}, \Theta\geq
   \theta_0)}{P(\Theta\geq \theta_0)} \leq  \frac{P(B_Z(\z, \theta_0 - \alpha_\varrho) \leq \alpha/{r_2}, \Theta' \geq
   \theta_0 - \alpha_\varrho)}{P(\Theta\geq \theta_0)}\\
   &=  \frac{P(B_Z(\z, \theta_0 - \alpha_\varrho) \leq \alpha/{r_2}, \Theta' \geq
   \theta_0 - \alpha_\varrho)}{P(\Theta' \geq
   \theta_0 - \alpha_\varrho)}\frac{P(\Theta' \geq
   \theta_0 - \alpha_\varrho)}{P(\Theta\geq \theta_0)}\\ 
   & \leq  P(B_Z(\z, \theta_0 - \alpha_\varrho) \leq \alpha/{r_2} \,|\, \Theta' \geq
   \theta_0 - \alpha_\varrho) \frac{P(\Theta \geq
   \theta_0 - \alpha_\varrho - \beta_\varrho)}{P(\Theta\geq
     \theta_0)}\\
  & \leq (\alpha/{r_2}) r_2 = \alpha\\
\end{align*}
\begin{align*}
& P(\{\mathrm{accept} \ H_0\} \ | \ H_1) = P(B_Z(\z, \theta_0 +
                 \beta_\varrho) \geq 1/\beta r_1 \ | \ H_1) =
                 P(B_Z(\z, \theta_0 + \beta_\varrho) \geq 1/\beta r_1
                 \ | \ \Theta < \theta_0)\\ 
 &=  \frac{P(B_Z(\z, \theta_0 + \beta_\varrho) \geq 1/\beta r_1,
   \Theta <
   \theta_0)}{P(\Theta < \theta_0)} \leq \frac{P(B_Z(\z, \theta_0 + \beta_\varrho) \geq 1/\beta r_1, \Theta' <
   \theta_0 + \beta_\varrho)}{P(\Theta < \theta_0)}\\
   &=  \frac{P(B_Z(\z, \theta_0 + \beta_\varrho) \geq 1/\beta r_1, \Theta' <
   \theta_0 + \beta_\varrho)}{P(\Theta' <
   \theta_0 + \beta_\varrho)}\frac{P(\Theta' <
   \theta_0 + \beta_\varrho)}{P(\Theta < \theta_0)}\\ 
   & \leq  P(B_Z(\z, \theta_0 + \beta_\varrho) \geq 1/\beta r_1 \,|\, \Theta' <
   \theta_0 + \beta_\varrho) \frac{P(\Theta <
   \theta_0 + \beta_\varrho + \alpha_\varrho)}{P(\Theta <
     \theta_0)}\\
  & \leq (1/\beta {r_1}) r_1 = 1/\beta\\
\end{align*}


% \begin{align*}
% & P(\{\mathrm{reject} \ H_0\} \ | \ H_0) = \\
%  &=  \frac{P(B_Z(\z, \theta_0 - \alpha_\varrho) \leq \alpha, \Theta' \geq
%    \theta_0 - \alpha_\varrho)}{P(\Theta\geq \theta_0)}\\
%    &=  \frac{P(B_Z(\z, \theta_0 - \alpha_\varrho) \leq \alpha, \Theta' \geq
%    \theta_0 - \alpha_\varrho)}{P(\Theta' \geq
%    \theta_0 - \alpha_\varrho)}\frac{P(\Theta' \geq
%    \theta_0 - \alpha_\varrho)}{P(\Theta\geq \theta_0)}\\ 
%    &\leq  \frac{P(B_Z(\z, \theta_0 - \alpha_\varrho) \leq \alpha, \Theta' \geq
%    \theta_0 - \alpha_\varrho)}{P(\Theta' \geq
%    \theta_0 - \alpha_\varrho)}\frac{P(\Theta \geq
%    \theta_0 - \alpha_\varrho - \beta_\varrho)}{P(\Theta\geq
%      \theta_0)}\\ 
%    &\leq  P(B_Z(\z, \theta_0 - \alpha_\varrho) \leq \alpha \,|\, \Theta' \geq
%    \theta_0 - \alpha_\varrho) r \\
% \end{align*}
%Similarly, we can show that $P(\{\mathrm{accept} \ H_0\}|H_1) \leq \beta$. 
	\end{proof}
%Note that $B_{Z}(\z, \theta_0+\beta') \leq B_{Z}(\z, \theta_0 -
%\alpha_\varrho)$. This implies that given a value of $\theta_0$,
%$\alpha'$ and $\beta'$, exactly one of the following holds: (a)
%$B_{Z}(\z, \theta_0+\beta') \geq \frac{1}{\beta'}$ (b) $B_{Z}(\z,
%\theta_0 - \alpha_\varrho) \leq \alpha'$ (c) neither (a) nor (b). \\

\textbf{Computation of $B_Z$:}         
        Theorem \ref{thm:yz} provides us a method to perform the
        hypothesis test on $\Theta$ using $Z$. This requires the
        computation of $B_Z$ that involves the $P_{Z|\Theta'}$ which
        is a Binomial distribution with parameter $\Theta'$ and
        $f_{\Theta'}$, the prior distribution for $\Theta'$.
        We do not know the exact distribution of $\Theta'$, however,
        we know that it is close to that of $\Theta$.
        We use this fact to obtain upper and lower bounds on the
        values of $B_Z$ and use that in the hypothesis test.


% We recall the Bayes' factor for the following hypothesis on $Z$:
% \vspace{-0.25cm}
% $$
% \vspace{-0.25cm}
% H_0': \Theta' \geq \theta_0'  \quad \text{vs} \quad H_1': \Theta'<\theta_0'
% $$
% \vspace{-0.25cm}
% $$
% \vspace{-0.15cm}
Bayes' factor for $Z$ given $\z$ and $\theta'_0$ is given by:
\[B_{Z}(\z,\theta_0') = \frac{\int_{\theta_0'}^1\P_{Z|\Theta'}(\z|\theta')\f_{\Theta'}(\theta')d\theta'}{\int_0^{\theta_0'}\P_{Z|\Theta'}(\z|\theta')\f_{\Theta'}(\theta')d\theta'}*\frac{\P_1}{\P_0}\]
where $\P_0 = \int_{\theta_0'}^1 \f_{\Theta'}(\theta')d\theta'$, $\P_1 = \int_0^{\theta_0'} \f_{\Theta'}(\theta')d\theta'$, and $\f_{\Theta'}(\theta')$ is a prior distribution of $Z$.
Note that exact computation of $B_{Z}$ is not possible because prior
distribution $\f_{\Theta'}$ of $Z$ is not known. Hence, we find the
lower and upper bound on $B_{Z}$ via  lower and upper bound on the
unknown prior distribution $\f_{\Theta'}$.

Let us assume that $\Theta'$ is a function of $\Theta$, say, $\Theta'
= g(\Theta)$ such that $- \alpha_\varrho \leq g(\Theta) - \Theta \leq
\beta_\varrho$. Note that this is a stronger assumption than $-
\alpha_\varrho \leq g(\Theta) - \Theta \leq \beta_\varrho$, however, a
reasonable assumption given this fact. (Our assumption requires that
an $\omega$ that map to $\theta$ through $\Theta$ maps to $g(\theta)$
through $\Theta'$.)
Further, let us assume that $g^{-1}$ is differentiable and its
derivative is bounded by some constants, $c \leq \frac{d}{d\theta'}g^{-1}(\theta') \leq
d$ for all $\theta' \in [0, 1]$.
Now, we can use transformation of random variables to obtain the pdf
$f_{\Theta'}$ of $\Theta'$.
\[f_{\Theta'}(\theta') = f_\Theta(g^{-1}(\theta'))
  \frac{d}{d\theta'}g^{-1}(\theta'),\]
and bound it using the derivate bounds:
\[  c  f_\Theta(g^{-1}(\theta')) \leq f_{\Theta'}(\theta')  \leq d  f_\Theta(g^{-1}(\theta')),\]
since, from our assumption,
$\frac{d}{d\theta'}g^{-1}(\theta') \in [c, d]$.
% \[c\frac{d}{d\theta'}g^{-1}(\theta') \leq f_{\Theta'}(\theta')  \leq d \frac{d}{d\theta'}g^{-1}(\theta')\]
Plugging $\Theta = g^{-1}(\theta')$ in $- \alpha_\varrho \leq
g(\Theta) - \Theta \leq \beta_\varrho$, 
we get $- \alpha_\varrho \theta' - g^{-1}(\theta') \leq
\beta_\varrho$. We can conclude
$\norm{\theta' - g^{-1}(\theta')} \leq \max\{\alpha_\varrho,
  \beta_\varrho\}$.

Suppose $f_\Theta$ is Lipschitz continuous with Lipschitz constant $L$,
that is,
$\norm{f_\Theta(\theta_1) - f_\Theta(\theta_2)} \leq L \norm{\theta_1
    - \theta_2}.$
Then,
$\norm{f_\Theta(\theta') - f_\Theta(g^{-1}(\theta'))} \leq L
  \norm{\theta' - g^{-1}(\theta')} \leq L \max\{\alpha_\varrho,
  \beta_\varrho\}$.
Hence,
$f_\Theta(\theta') - L \max\{\alpha_\varrho,
  \beta_\varrho\} \leq f_\Theta(g^{-1}(\theta')) \leq
  f_\Theta(\theta') + L \max\{\alpha_\varrho,
  \beta_\varrho\}$. Therefore,
\[ c (f_\Theta(\theta') - L \max\{\alpha_\varrho, \beta_\varrho\}) \leq
  f_{\Theta'}(\theta') \leq  d  (f_\Theta(\theta') + L \max\{\alpha_\varrho,   \beta_\varrho\})\] 


We can compute upper and lower bounds on $B_Z(\z, \theta')$ as in the
next proposition.

\begin{proposition}
		\label{prop3}
		Let $Y\sim \Bd(\Theta)$ and  $Z \sim \Bd(\Theta')$ be
                Bernoulli random variables with parameter $\Theta$ and
                $\Theta'$, respectively, and let  Equation
                \ref{eqn:error} hold.
                Assume $Z = g(Y)$, where $g^{-1}$ is differentiable
                and in the range $[c, d]$.
                Let $f_\Theta$ be Lipschitz continuous with Lipschitz
                constant $L$. 
                Let $\gamma = L \max\{\alpha_\varrho,
                \beta_\varrho\}$. Let
$$
B_Z(\z,\theta_0')_{min} = \frac{c^2}{d^2}*\frac{\P_1^{min}}{\P_0^{max}}
*\frac{\int_{\theta_0'}^1(\theta')^{m}(1-\theta')^{(n-m)}(f_{\Theta}(\theta')-
  \gamma)d\theta'}{\int_0^{\theta_0'}(\theta')^{m}(1-\theta')^{(n-m)}(f_{\Theta}(\theta')+\gamma)d\theta'}
$$
	\vspace{-0.15cm}
$$
	B_Z(\z,\theta_0')_{max} = \frac{d^2}{c^2}*\frac{\P_1^{max}}{\P_0^{min}}* \frac{\int_{\theta_0'}^1(\theta')^{(m)}(1-\theta')^{(n-m)}(f_{\Theta}(\theta')+\gamma)d\theta'}{\int_0^{\theta_0'}\theta'^{(m)}(1-\theta')^{(n-m)}(f_{\Theta}(\theta')-\gamma)d\theta'}, \ \mathrm{	where }
	$$
		\vspace{-0.20cm}
	$$
	\vspace{-0.15cm}
	\P_0^{min} = \int_{\theta_0'}^1 (\f_{\Theta}(\theta')-\gamma)d\theta', \P_0^{max} = \int_{\theta_0'}^1 (\f_{\Theta}(\theta')+\gamma)d\theta',$$
	$$
	\P_1^{min} = \int_0^{\theta_0'}
        (\f_{\Theta}(\theta')-\gamma)d\theta', \P_1^{max} =
        \int_0^{\theta_0'} (\f_{\Theta}(\theta')+\gamma)d\theta',$$
        $m=\sum_{i=1}^n z_i$ and $n$ is the sample size of $\z$.
	Then, we have 
		\vspace{-0.15cm}
	$$ 	\vspace{-0.15cm}
	B_Z(\z,\theta_0')_{min}\leq B_Z(\z,\theta_0') \leq B_Z(\z,\theta_0')_{max}.$$
\end{proposition}

The following proposition states that Beta distribution is a Lipschitz
continuous function.
\begin{proposition}
	\label{prop2}
	Let $\f_{\Theta}$ be a Beta prior distribution for  fixed
        shape parameters $a$, $b$, that is, $ 
	\f_{\Theta}(\theta) = \frac{\theta^{a}
          (1-\theta)^b}{Beta(a,b)}, \ \mathrm{for} \ 0 \leq \theta
        \leq 1$. 	Then $f_\Theta$ is a Lipschitz continuous
        function with Lipschitz constant $L = \frac{(a+b)}{Beta(a,b)}$.
	\end{proposition}



        %%% ALGORITHM NESTED

\section{Bayesian SMC Algorithm for Nested CSL}
Algorithm \ref{algo:nested} describes the verification of a CSL
formula $\varphi = \Pr_{\op \theta_0}(\rho)$, where $\rho$ could
potentially have nested probabilistic operators.
If $\rho$ is non-nested, then the algorithm calls the Bayesian SMC for
the non-nested case.
If $\rho$ is a nested formula, $\alpha_\varrho, \beta_\varrho \in (0,
1)$ are chosen such that $\theta_0 - \alpha_\varrho, \theta_0 + \beta_\varrho \in (0,
1)$. We leave the exact procedure to be figured out during the
implementation, as it does not affect the correctness of the
algorithm.

\compute($\varrho$,$\alpha_\varrho$, $\beta_\varrho$) returns (a
vector of) error bounds $\alpha_\psi, \beta_\psi$ for all top-level
formula $\psi$ such that $\alpha_\varrho, \beta_\varrho$ are upper
bounds on the errors propagated from the top-level formulae $\psi$ to
$\rho$ using the error propagation rules in Section \ref{sec:error}.
The Bayesian SMC algorithm is called recursively on each top-level
formula $\psi$ and state $s'$ of the DTMC $\T$ to obtain the ``truth''
values $t_{\psi, s'}$ with guaranteed error bounds $\alpha_\psi,
\beta_\psi$.

$\rho$ is then treated as a ``non-nested'' formula where each top
level formula $\psi$ is treated as a proposition with truth value
$t_{\psi, s'}$ in state $s'$.
Let $L_\rho$ be the depth of this ``non-nested'' formula.
Samples $\sigma$ of length $L_\rho$ are generated, and $\sigma \models
\rho$ is checked using the computed values $\{t_{\psi, s'}\}$.
$n$ is the total number of samples and $m$ the number of samples that
satisfy $\rho$ as above.
BayesFactorMin and BayesFactorMax implement $B_Z(\z, \theta')_{min}$
and $B_Z(\z, \theta')_{max}$, respectively.
ProbBounds computes $r_1$ and $r_2$ from Theorem \ref{thm:yz}; lower
and upper bounds on $B_Z$ are used to check the acceptance/rejection
conditions in the theorem.

        \begin{algorithm}[h] 
	\vspace{2 mm}
	\KwIn{$s$ - state, $\T$ - $\mc$, $\varphi = \Pr_{\op \theta_0}
          (\rho)$ - (nested) $\csl$ formula, $a$, $b$ - parameters
          for beta prior, $\alpha$, $\beta$ - bound on Type I and Type
          II errors, assumption constants $c, d$
	}
	\vspace{2 mm}
	\KwOut{Answer if $s \models \varphi$ in $\T$ with confidence
          $\alpha, \beta$ }
	\vspace{2 mm}
	\caption{Bayes$\_$SMC$\_$Nested - SMC of a non-nested $\csl$
          formula}
	\label{algo:nested}
	\SetKw{KwGoTo}{go to}
	\Begin{ 	 
  	\If{$\varphi$ is nested $\csl$ formula}
        {
          Compute $\alpha_\varrho, \beta_\varrho \in (0, 1)$ such that
          $\theta_0 - \alpha_\varrho, \theta_0 + \beta_\varrho \in (0,
          1)$

          $\bar{\alpha}$, $\bar{\beta}$ = \compute($\varrho$,
          $\alpha_\varrho$, $\beta_\varrho$)

          \For{$\psi$ in $\next(\varphi)$ and state $s'$ of $\T$}{
		
		$t_{\psi,s'}$ = Bayes$\_$SMC$\_$Nested($s'$, $\T$,
                $\psi$, $a$, $b$, $\alpha_\psi$, $\beta_\psi$, $c$, $d$)		
		} 
          Set $n = 0$, $m = 0$\\
          Set $\lenf{\varrho}$ to be the depth of (non-nested part of)
          $\varrho$\\
          
		\While{True}
		{
			Increment $n$\\
			Generate a (random) path $\sigma$ from state $s$ in
                        $\T$ of length $\lenf{\varrho}$ \\
			\If{$\sigma$ satisfies $\rho$ using $\{t_{\psi,
                          s'}\}$} {
				Increment $m$
			}
				Set $B_{min}$ =
                                BayesFactorMin($\theta_0 + \beta_\varrho$,
                                $n$, $m$, $a$, $b$, $\alpha_\varrho$, $\beta_\rho$, $c$, $d$) \\
				Set $B_{max}$ =
                                BayesFactorMax($\theta_0 - \alpha_\varrho$,
                                $n$, $m$, $a$, $b$, $\alpha_\varrho$,
                                $\beta_\rho$, $c$, $d$) \\

                                Set $r_1, r_2$ = ProbBounds($\theta_0$,
                                $a$, $b$, $\alpha_\varrho$, $\beta_\rho$)

			\If{$B_{min} > \frac{1}{r_1\beta}$}
			{
				\textbf{return} \emph{true}		
			}
			\If{$B_{max} < \alpha/r_2$}{
				\textbf{return} \emph{false}		
			}	
		}



              }
		\Else{
			\Return Bayes$\_$SMC$\_$Base($s$, $\T$, $\varphi$, $a$, $b$, $\alpha$, $\beta$) 		
		} 	
	}		 

        
	% \label{algo:base}
	% \SetKw{KwGoTo}{go to}
	% \Begin{ 	 
        %   Set $n = 0$, $m = 0$\\
        %   Set $\lenf{\varrho}$ to be the depth of $\varrho$\\
          
	% 	\While{True}
	% 	{
	% 		Increment $n$\\
	% 		Generate a (random) path $\sigma$ from state $s$ in
        %                 $\T$ of length $\lenf{\varrho}$ \\
	% 		\If{$\sigma$ satisfies $\rho$} {
	% 			Increment $m$
	% 		}
	% 			Set $B$ = BayesFactor($\theta_0$, $n$, $m$, $a$, $b$) \\
	% 		\If{$B > \frac{1}{\beta}$}
	% 		{
	% 			\textbf{return} \emph{true}		
	% 		}
	% 		\If{$B < \alpha$}{
	% 			\textbf{return} \emph{false}		
	% 		}	
	% 	}
	
	% }		 
      \end{algorithm}



%         According to lower and upper bound on $B_Z(\z,\theta_0')$, we can conclude about the test on $Z$ via lower and upper bound on the Bayes' factor of $B_Z$ because when $B_Z(\z,\theta_0')_{min}\geq \frac{1}{\beta}$, we have $B_Z(\z,\theta_0') \ge \frac{1}{\beta}$, and when $B_Z(\z,\theta_0')_{max} \leq \alpha$, we have $B_Z(\z,\theta_0') \leq \alpha$ for a given Type I and Type II error bound $\alpha$, $\beta$, respectively. 

% We use $B_{Z}(\z, \theta_0+\beta')_{min}$ and $B_{Z}(\z, \theta_0 - \alpha_\varrho)_{max}$ in place of $B_{Z}(\z, \theta_0+\beta')$ and $B_{Z}(\z, \theta_0 - \alpha_\varrho)$, respectively, in Theorem \ref{thm2}. 
% The Theorem \ref{thm2} will still hold because $ B_{Z}(\z, \theta_0+\beta') \geq B_{Z}(\z, \theta_0+\beta')_{min} \geq \frac{1}{\beta}$, and $B_{Z}(\z, \theta_0 - \alpha_\varrho) \leq B_{Z}(\z, \theta_0 - \alpha_\varrho)_{max} \leq \alpha$.
% %Next, we present an algorithm for the verification of a nested $\csl$ formula.


% In this section, we present algorithms for testing nested $\csl$ formula $\varphi$ on a DTMC $\T$. In Algorithm \ref{algo:nested}, we recursively deduce from a nested $\csl$ formula to a non-nested $\csl$ formula based on verification results of the top formula at each state of $\T$. Then, Algorithm \ref{algo:nonnested} is used for testing of the non-nested $\csl$ formula, which is similar to as given in the paper~\cite{zuliani2010bayesian}.
% %For Algorithm \ref{algo:nonnested}, we have fixed the bound on Type I error  and Type II error as $\alpha$, $\beta$ for each non-nested $\csl$ formula.
% Next, we describe the details of Algorithms \ref{algo:nested},
% \ref{algo:nonnested}.

% \begin{algorithm}[h] 
% 	\vspace{2 mm}
% 	\KwIn{$s$ - state, $\T$ - $\mc$, $\varphi$ - $\csl$ formula, $a$, $b$ - parameters for beta prior, $\alpha$, $\beta$ - bound on Type I and Type II error, $\alpha'$, $\beta'$ - Propagated error, $P(Z=1|Y=0) \leq \beta'$,
% 		% $\alpha'$, $\beta'$ - bound on probability of error in making decision, that is, $Pr(Z=1|Y=0)$, $Pr(Z=0|Y=1)$, respectively, 
% 		$L$ - length of path
% 	}
% 	\vspace{2 mm}
% 	\KwOut{Accept/Reject the whole $\csl$ formula}
% 	\vspace{2 mm}
% 	\caption{Verify$\_$CSL - testing of the nested $\csl$ formula}
% 	\label{algo:nested}
% 	\SetKw{KwGoTo}{go to}
% 	\Begin{ 	 
% 		Let $\varphi = \Pr_{\op \theta_0} (\varrho)$ \\
% 		\If{$\varphi$ is nested $\csl$ formula}
% 		{
% 			\For{$\psi$ in $\next(\varphi)$}{
% 				$\alpha_{\psi}$, $\beta_{\psi}$ = \compute($\varphi$, $\alpha'$, $\beta'$) 		[From Property \ref{r:1}]
% 			}		
% 			\For{$\psi$ in $\next(\varphi)$ and state $s'$ of $\T$}{
% 				Let $\psi = \Pr_{\op \theta_0'}$($\psi'$) \\
% 				$t_{\psi,s'}$ = Verify$\_$CSL($s'$, $\T$, $\psi$, $a$, $b$, $\alpha$, $\beta$,
% 				$\alpha_{\psi}$, $\beta_{\psi}$, $L$)		
% 			} 
			
% 			\For{$\psi$ in $\next(\varphi)$}{
% 				$\varphi$ = \replace($\varphi$, $\psi$, $\{t_{\psi,s'}\}_{s' \in \S}$)
% 			}
			
% 			\textbf{return}	Bayes$\_$Verify($s$, $\T$, $\varphi$,  $a$, $b$, $\alpha$, $\beta$, $\alpha'$, $\beta'$, $L$)  \\				
% 		}
% 		\Else{
% 			$t_{\varphi,s}$ = Bayes$\_$Verify($s$, $\T$, $\varphi$, $a$, $b$, $\alpha$, $\beta$, $0$, $0$, $L$) 		
% 		} 	
% 	}		 
% \end{algorithm}
% \vspace{-0.50cm}
% In Algorithm \ref{algo:nested}, first, we check whether the formula $\varphi$ is nested at line $3$. If it is nested, then we propagate the error to the top formula of  $\varphi$ in  in lines $3-4$ via $compute\_error$ function, which performs error distribution according to Property \ref{r:1}. In lines $6-8$, we call the same Algorithm \ref{algo:nested} for each top formula $\psi$. If $\psi$ is nested $\csl$, then we repeat lines $4-8$ for it. Otherwise, we call Algorithm \ref{algo:nonnested} at line $13$ for testing of $\psi$ at each state of $\T$.
% Once, we have verification results for each top formula $\psi$, we replace each top formula $\psi$ of $\varphi$ with a propositional formula  which is a conjunction of boolean variables $t_{\psi,s'}$ for those states $s'$ at which $\psi$ is true at lines $9-10$ where the evaluation of $t_{\psi,s'}$ can be true/false based on the test result of $\psi$ . After replacement, the formula $\varphi$ becomes a non-nested $\csl$ formula.  Then, we call Algorithm \ref{algo:nonnested} for testing $\varphi$ at line $11$.



% %In Algorithm \ref{algo:nonnested}, we first generate a sample path $\sigma$ at line $6$, and check whether $\sigma$ satisfies the temporal logic $\phi$ of the non-nested $\csl$ formula $\varphi$. If it satisfies, then we increase the number of satisfied samples by $1$ at line $8$. 
% %In line $9$, we compute Bayes' factor according to Proposition \ref{prop3}. Then, we either conclude the test based on the value of Bayes' factor at lines $10-13$ or repeat the loop until the number of generated samples are enough to conclude the test. Next, we present the experimental evaluation of our method.

% \begin{algorithm}[h] 
% 	\vspace{2 mm}
% 	\KwIn{$s$ - state, $\T$ - $\mc$, $\varphi$ - $\csl$ formula, $a$, $b$ - parameters for beta prior, 
% 			$\alpha$, $\beta$ - bound on Type I and Type II error, $\alpha'$, $\beta'$ - error bound between $Y$ and $Z$, that is, $P(Z=0|Y=1) \leq \alpha'$, $P(Z=1|Y=0) \leq \beta'$
% 	%	$\alpha'$, $\beta'$ -  bound on probability of error in making decision, that is, $Pr(Z=1|Y=0)$, $Pr(Z=0|Y=1)$, respectively, 
% 		$L$ - length of path
% 	}
% 	\vspace{2 mm}
% 	\KwOut{Accept/Reject the $\csl$ formula}
% 	\vspace{2 mm}
% 	\caption{Bayes$\_$Verify - testing of a non-nested $\csl$ formula}
% 	\label{algo:nonnested}
% 	\SetKw{KwGoTo}{go to}
% 	\Begin{ 	 
% 		Let $\varphi = \Pr_{\op \theta_0} (\phi)$; 	n=0, m=0 \\
% 		\While{True}
% 		{
% 			n =n+1 \\
% 			Generate a path $\sigma$ from state $s$ with length $L$ \\
% 			\If{$\sigma$ satisfies $\phi$} {
% 				m = m+1			
% 			}
% 				$B_{min}$, $B_{max}$ = Bayesfactor($\theta_0$, $n$, $m$, $a$, $b$, $\alpha'$, $\beta'$) [From Proposition \ref{prop3}]\\
% 			\If{$B_{min} > \frac{1}{\beta}$}
% 			{
% 				\textbf{return} \emph{true}		
% 			}
% 			\If{$B_{max} < \alpha$}{
% 				\textbf{return} \emph{false}		
% 			}	
% 		}
	
% 	}		 
% \end{algorithm}
 
% %
% %\section{Bayesian Statistical Model-Checking Algorithm}
% %\label{sec:algo}
% %In this section, we present algorithms for testing nested $\csl$ formula based on the testing method given above. The details of the algorithm are given as follows.
% %
% %\begin{flushleft}
% %	\begin{figure*}
% %		\hfill
% %		\subfigure[$\mc$ $\T$ \label{fig:sys}]{\includegraphics[width=3.5cm, height=4.2cm]{image/sys.pdf}}
% %		\hfill
% %		\subfigure[ $ Pr_{\geq 0.1}(Pr_{\geq 0.2}(F^{\leq 1} b) U^{\leq 4} g)$ \label{fig:f}]{\includegraphics[width=3.5cm, height=4.2cm]{image/ex1.pdf}}
% %		\hfill
% %		\subfigure[ $ Pr_{\geq 0.1}(((s_0 \lor s_2 \lor s_3)\land \neg s_1) U^{\leq 4} g)$ \label{fig:subf}]{\includegraphics[width=4.0cm, height=3cm]{image/ex2.pdf}}
% %		\hfill
% %		\caption{Example}
% %	\end{figure*}
% %\end{flushleft}
% %
% %\begin{algorithm}[h] 
% %	
% %	\vspace{2 mm}
% %	\KwIn{$s$ - state, $\T$ - $\mc$, $\varphi$ - $\csl$ formula, $\theta_0$ - outer probability threshold in $\varphi$, $a$, $b$ - parameters for beta prior, $\alpha$, $\beta$ - probability of Type I and Type II error, $L$ - length of path, $flag$ - $\top/\bot$ based on non-nested/nested formula
% %	}
% %	\vspace{2 mm}
% %	\KwOut{Accept/Reject the $\csl$ formula}
% %	\vspace{2 mm}
% %	\caption{Bayes-verify$\_$CSL - testing of $\csl$ formula}
% %	\label{algo:nonnested}
% %	\SetKw{KwGoTo}{go to}
% %	\Begin{ 	 
% %		Let $\varphi = \Pr_{\geq \theta_0} (\varrho)$ \\
% %		n=0, m=0 \\
% %		\While{True}
% %		{
% %			n =n+1 \\
% %			Generate a path $\sigma$ from state $s$ with length $L$ \\
% %			\If{$\sigma$ satisfies $\varrho$} {
% %				m = m+1			
% %			}
% %			\If{flag=$\top$}{
% %				$B_{min}$, $B_{max}$ = Bayesfactor($\theta_0$, $n$, $m$, $a$, $b$, 0, 0)
% %			}
% %			\Else{
% %				$B_{min}$, $B_{max}$ = Bayesfactor($\theta_0$, $n$, $m$, $a$, $b$, $\alpha$, $\beta$)
% %			}
% %			\If{$B_{min} > \frac{1}{\alpha}$}
% %			{
% %				\textbf{return} \emph{true}		
% %			}
% %			\If{$B_{max} < \beta$}{
% %				\textbf{return} \emph{false}		
% %			}	
% %		}
% %	}		 
% %\end{algorithm}
% %
% %
% %
% %The Algorithm \ref{algo:nonnested} takes following parameters as input: state - $s$, $\mc$ $\mathcal{T}$, nested $\csl$ formula $\varphi$,  outer probability threshold  $\theta_0$ in $\varphi$, prior parameters $a$ and $b$, upper bound on probability of Type I and Type II  error $\alpha$ and $\beta$,  length of path $L$,  and returns \emph{true} if $\varphi$ is accepted and \emph{false} otherwise.  We perform the following steps in iterative fashion. First, we generate a random sample path $\sigma$ with length $L$ which can be expressed as a Bernoulli variable $Y$ with parameter $\Theta = \prob(\C_{\varrho,L})$ according to Section \ref{sec:nonnested}.  We then compute the minimum and the maximum Bayes' factor $B_{min}$, $B_{max}$ at line 10 and line 12 according to Equations \ref{eqn:bmin}, \ref{eqn:bmax}. Note that if  $\varrho$ has no probabilistic operator in there, $B_{min}$, $B_{max}$ are the same as  Bayes' factor computed from Equation \ref{eqn:b}.  Given value of $B_{min}$, $B_{max}$, the decision is made  based on so far generated random paths from lines 13-16.
% %We repeat the process until the decision is made about either acceptance or rejection of $\varphi$.
% %
% %
% %Algorithm \ref{algo:nested} is the recursive algorithm to test the whole $\csl$ formula. It takes following parameters as input: state - $s$, $\mc$ $\mathcal{T}$, nested $\csl$ formula $\varphi$,  outer probability threshold  $\theta_0$ in $\varphi$, beta prior parameters $a$ and $b$, upper bound on probability of Type I and Type II  error $\alpha$ and $\beta$,  length of path $P$, and returns \emph{true} if $\varphi$ is accepted and \emph{false} otherwise. Next, we provide the details about 
% %Algorithm \ref{algo:nested}.
% %
% %In Algorithm \ref{algo:nested}, we first check whether the formula $\varphi$ is nested $\csl$ at line $3$. If so, we propagate the upper bound of Type I and Type II error to the top level probabilistic subformula of $\varphi$ using \compute$ $ function at lines 4-5. Then, we recursively test each top level probabilistic subformula $\psi$ for each state of $\T$ and propagated upper bound on Type I and Type II error $\alpha_{\psi}$, $\beta_{\psi}$, respectively, at lines 6-8. When we have the status about each top level  probabilistic subformula returned by the recursive calls at line 8, we replace top level subformula $\psi$ in $\phi$ by a propositional formula which captures the satisfaction of $\psi$ over the states of $\T$ at lines 9-10. In other words,  the propositional formula is disjuction of all those states $s'$s for which $t_{\psi,s'}$ is true. Now, the formula $\varphi$ is a state formula. Hence, we call Algorithm \ref{algo:nonnested} to check the acceptance or rejection of the formula $\varphi$. Furthermore, we explain each step in Algorithm  \ref{algo:nested}  via a running example.
% %
% %Consider $\mc$ $\T$ shown in Figure $\ref{fig:sys}$, where the set of atomic propositions are $\{s_0, s_1, s_2,s_3, r, b, g\}$, that is, states are included in the atomic proposition.  Let a nested $\csl$ formula $\varphi$ be $Pr_{\geq 0.1}[Pr_{0.2}(F^{\leq 1}g) U^{\leq 4} g]$ whose parse tree is shown in Figure \ref{fig:f}. We illustrate Algorithm \ref{algo:nested} for beta prior parameters $a=b =1$, upper bound on the probability of Type I and Type II error $\alpha=\beta = 0.05$, and length of path $P=4$.  At line 2, $\varphi = Pr_{\geq 0.1} (\phi)$, where $\phi = [Pr_{0.2}(F^{\leq 1}g) U^{\leq 4} g]$. In this formula $\varphi$, there is only one top level subformula $\psi = [Pr_{\geq 0.2} F^{\leq 1} b]$ which is circled in Figure \ref{fig:f}. Then, we propagate the errors $\alpha$, $\beta$ for the subformula $\psi$ at lines 4-5 and the propagation of the errors is computed by Algorithm \ref{algo:compute}. Here, we obtain propagated errors $\alpha_{\psi} = \frac{1}{20}$, $ \beta_{\psi} = \frac{1}{100}$ for $\psi$. Then, for each state $s'$ of $\T$, we call Algorithm \ref{algo:nonnested} for the acceptance or rejection of $\psi$ which returns either \emph{true} or \emph{false} which is saved in $t_{\psi,s'}$ at lines 6-10.  Here, we obtain 
% %$t_{\psi,s_0} = t_{\psi,s_2} = t_{\psi,s_3} = \top$ and $t_{\psi,s_1} = \bot$. Then, we reduce the formula $\phi$ into a state formula based on the test results for $\psi$ at lines 9-10. We basically replace the formula $\psi$ by the  propositional formula $[(s_0 \lor s_2 \lor s_3) \wedge \neg s_1]$ which is constructed based on values of $t_{\psi, s'}$. Now, the formula $\phi$ becomes $((s_0 \lor s_2 \lor s_3) \land \neg s_1) U^{\leq 4} g$, that is, $\varphi = Pr_{\geq 0.1}[((s_0 \lor s_2 \lor s_3) \land \neg s_1) U^{\leq 4} g]$ as shown in Figure \ref{fig:subf}. We then call  Algorithm \ref{algo:nonnested} to test the acceptance or rejection of $\varphi$.
% %
% %\begin{algorithm}[h] 
% %	
% %	\vspace{2 mm}
% %	\KwIn{$s$ - state, $\T$ - $\mc$, $\varphi$ - $\csl$ formula, $\theta_0$ - outer probability threshold in $\phi$, $a$, $b$ - parameters for beta prior, $\alpha$, $\beta$ - probability of Type I and Type II error,
% %		$P$ - length of path
% %	}
% %	\vspace{2 mm}
% %	\KwOut{Accept/Reject the whole $\csl$ formula}
% %	\vspace{2 mm}
% %	\caption{Recursive-verify$\_$CSL - testing of the whole $\csl$ formula}
% %	\label{algo:nested}
% %	\SetKw{KwGoTo}{go to}
% %	\Begin{ 	 
% %		Let $\varphi = \Pr_{\geq \theta_0} (\phi)$ \\
% %		\If{$\varphi$ is nested $\csl$ formula}
% %		{
% %			\For{$\psi$ in $\next(\varphi)$}{
% %				$\alpha_{\psi}$, $\beta_{\psi}$ = \compute($\varphi$, $\alpha$, 
% %				$\beta$) 		
% %			}		
% %			\For{$\psi$ in $\next(\varphi)$ and state $s'$ of $\T$}{
% %				Let $\psi = \Pr_{\op \theta_0'}$($\psi'$) \\
% %				$t_{\psi,s'}$ = Recursive-verify$\_$CSL($s'$, $\T$, $\psi$, $\theta_0'$, $a$, $b$, 
% %				$\alpha_{\psi}$, $\beta_{\psi}$, $P$)		
% %			} 
% %			
% %			\For{$\psi$ in $\next(\varphi)$}{
% %				$\phi$ = \replace($\psi$, $\{t_{\psi,s'}\}_{s' \in \S}$)
% %			}
% %			
% %			\textbf{return}	Bayes-verify$\_$CSL($s$, $\T$, $\varphi$, $\theta_0$, $a$, $b$, $\alpha$, $\beta$, $P$, $\bot$)  \\				
% %		}
% %		\Else{
% %			$t_{\varphi,s}$ = Bayes-verify$\_$CSL($s$, $\T$, $\varphi$, $\theta_0$, $a$, $b$, $\alpha$, $\beta$, $P$, $\top$) 		
% %		} 	
% %	}		 
% %\end{algorithm}
% %
% %
% %Next, we introduce Algorithm \ref{algo:compute} for the propagation of errors to the top level subformula of a given $\csl$ formula $\varphi$ and upper bound on Type I and Type II error $\alpha$, $\beta$, respectively. The details of Algorithm \ref{algo:compute} comes from Property \ref{r:1}.
% %
% %
% %\begin{algorithm}[h] 
% %	
% %	\vspace{2 mm}
% %	\KwIn{ nested $\csl$ formula - $\varphi$,  upper bound on Type I and Type error - $\alpha$, $\beta$}
% %	\vspace{2 mm}
% %	\KwOut{$\alpha_{\psi}, \beta_{\psi}$ - propagation of errors for each top level probabilistic subformula $\psi$}
% %	\vspace{2 mm}
% %	\caption{\compute - propagation of errors to top level  probabilistic subformula of $\varphi$}
% %	\label{algo:compute}
% %	\SetKw{KwGoTo}{go to}
% %	\Begin{ 	 
% %		Let $\varphi = \Pr_{\geq \theta_0} (\phi)$ \\
% %		\If{$\phi = \neg(\psi)$} {
% %			$\alpha_{\psi} = \beta$, $\beta_{\psi} = \alpha$
% %		}
% %		\If{$\phi = \psi_1 \land \psi_2$}{
% %			$\alpha_{\psi_1} = \alpha_{\psi_2} =\frac{\alpha}{2}$, $\beta_{\psi_1} = \beta_{\psi_2} = \beta$
% %		}	 
% %		\If{$\phi = X\psi$}{
% %			$\alpha_{\psi} = \alpha$, $\beta_{\psi} = \beta$
% %		}			
% %		\If{$\phi = \psi_1 U^{\leq k} \psi_2$}{
% %			$\alpha_{\psi_1} = \alpha_{\psi_2} =\alpha$, $\beta_{\psi_1} = \beta_{\psi_2} = \frac{\beta}{k+1}$
% %		}
% %	}		 
% %\end{algorithm}

